The Deep Bootstrap Framework: Good Online Learners are Good Offline Generalizers

We propose a new framework for reasoning about generalization in deep learning. The core idea is to couple the Real World, where optimizers take stochastic gradient steps on the empirical loss, to an Ideal World, where optimizers take steps on the population loss. This leads to an alternate decomposition of test error into: (1) the Ideal World test error plus (2) the gap between the two worlds. If the gap (2) is universally small, this reduces the problem of generalization in offline learning to the problem of optimization in online learning. We then give empirical evidence that this gap between worlds can be small in realistic deep learning settings, in particular supervised image classification. For example, CNNs generalize better than MLPs on image distributions in the Real World, but this is "because" they optimize faster on the population loss in the Ideal World. This suggests our framework is a useful tool for understanding generalization in deep learning, and lays a foundation for future research in the area.

==> sec_scratch.tex <==
\section{Outline (scratch)}
\pnote{for our own organization}

Main Experiments:
\begin{enumerate}
\item Zeroth-order claim: $|\eps|$ small ($< 3\%$ for $n=50K$, $< 7\%$ for $n > 5K$).
\begin{enumerate}
    \item CIFAR-5m sweep varying architecture, nsamps, aug for realistic models: to establish zeroth-order claim that $|\eps|$ is small.
    \item (random-NAS sweep: sampling 1000s of random NAS architectures for n=50K samples).
    \item (ImageNet experiments?)
\end{enumerate}
\item First-order investigations
\begin{enumerate}
\item Sample size
\item Stopping-time $T$
\item Data-augmentation
\item Learning-rate
\item Model size
\item pretraining 
\item (batch-size?)
\end{enumerate}
\end{enumerate}



\section{Scratch Work}
Our approach could apply to any setting where an iterative optimizer for online learning (e.g. stochastic gradient descent) is applied in an offline setting,
though in this work we specifically consider gradient-based optimizers
applied to deep neural networks for image classification.
This is an appropriate domain to vet theories of generalization,
since it is well-developed in practice, thoroughly studied in theory,
and yet continues to have a large gap between theory and practice.


Our central claim is that in realistic deep learning settings,
the classifiers output in the Real and Ideal worlds are close in meaningful ways.
Specifically, they are close in test soft-error (i.e. test error of temperature-1 samples from the model).


Since standard classification tasks (e.g. CIFAR-10)
do not have enough samples to construct the corresponding Ideal World,
we construct several datasets to serve as proxies.
For CIFAR-10, we construct a dataset of 5 million ``CIFAR-like'' samples,
created by by a CIFAR-10 generative model \citep{ho2020denoising}
labeled by a good CIFAR-10 classifier (BigTransfer-M).
These samples are realistic enough for our purposes
to serve as a proxy for CIFAR-10 (details are in Section?).


\subsection{Significance}
One of the most basic yet fundamental open questions in the theory of machine learning
is to theoretically understand why supervised deep learning works ---
that is, why training large neural networks with gradient-based methods yield classifiers with small test error.
In theory, we hope for a bound on the test error of trained classifiers
which is correct, non-vacuous, and predictive: we hope that this bound can
justify and inform important practical design choices such as architecture, optimizer,
number of samples, etc.

Many works have attempted to attack this question, often by adapting classical tools
(e.g. uniform convergence, stability, margins) to deep neural networks.
However, most if not all of this work currently falls short of being non-vacuous and predictive.
The gap between theory and practice is most extreme for \emph{interpolating} methods,
which fit their train sets exactly, leading to a recent surge in research on interpolating methods \citep{...}.

These prior works use different techniques under the hood, but they ultimately try to
understand the test error via bounding the \emph{generalization gap}.
That is, they decompose the test error into (1) train error plus (2) generalization gap,
and then attempt to bound the generalization gap.
Interpolating methods pose challenges to this approach, since the generalization gap
can be high -- there is in fact a difference between the train and test errors.



